Temporal models for demographic and global health outcomes in multiple populations: Introducing a new framework to review and standardize documentation of model assumptions and facilitate model comparison

There is growing interest in producing estimates of demographic and global health indicators in populations with limited data. Statistical models are needed to combine data from multiple data sources into estimates and projections with uncertainty. Diverse modeling approaches have been applied to this problem, making comparisons between models difficult. We propose a model class, Temporal Models for Multiple Populations (TMMPs), to facilitate documentation of model assumptions in a standardized way and comparison across models. The class distinguishes between latent trends and the observed data, which may be noisy or exhibit systematic biases. We provide general formulations of the process model, which describes the latent trend of the indicator of interest. We show how existing models for a variety of indicators can be written as TMMPs and how the TMMP-based description can be used to compare and contrast model assumptions. We end with a discussion of outstanding questions and future directions.

==> tables/data_model.tex <==
\begin{tabularx}{1\textwidth}{
        |>{\raggedright\arraybackslash}X
        |>{\raggedright\arraybackslash}X
        |>{\raggedright\arraybackslash}X
        |>{\raggedright\arraybackslash}X
        |>{\raggedright\arraybackslash}X
        |>{\raggedright\arraybackslash}X
        |>{\raggedright\arraybackslash}X
        |>{\raggedright\arraybackslash}X |
    }
    
    \hline
                      & Alexander 2018 NMR     & Cahill 2018 FP & GBD U5MR & Alkema and New 2014 U5MR & Alkema 2017 MMR & BMat 2019 \\
    \hline
    
    
    Response model $\pi_i$     & normal             & normal      & normal  & normal, $t$-distribution & normal & normal \\
    
    \hline
    
    Data transformation $f_{1,i}$    & log                & log-ratio   & log  & log & log & log \\
    
    \hline
    
    Process model transformation parameters $\bm{\gamma}$ & & & & & & $\gamma_{i, 1}, \gamma_{i, 2}$ \\
    
    \hline
    
    Process model transformation $f_{2,i}$             &                 &    &  &  &  & $\log(\eta_{i}) + (\gamma_{i, 1} + \gamma_{i, 2})I(\text{obs $i$ is pregn related})$ \\
    
    \hline
    
    Variance parameters $\bm{\sigma}_i$ & & & & & & $\sigma^2_{d[i]}$ \\
    
    \hline
    
    Fixed variance inputs & & & & & & $s_i^2$ \\
    
    \hline
    
    Variance function $f_{3,i}(\bm{\sigma}_i)$            &                &   &  & & non-VR data: $s_i^2 + \sigma^2_{d[i]}$ & non-VR data: $s_i^2 + \sigma^2_{d[i]}$ \\
    
    \hline
    
    
    Sampling error             & fixed              & estimated   & fixed & fixed, estimated  & fixed & \\
    
    \hline
    
    Non-sampling error            & estimated          & estimated & fixed & estimated & estimated & \\
    
    \hline
    
    Systematic bias  & no & estimated & no & estimated & fixed, estimated  & \\
    
    \hline
    
    
\end{tabularx}

==> tables/gbd_igme_comparison.tex <==
\begin{tabularx}{1\textwidth}{
        |>{\raggedright\arraybackslash}X
        |>{\raggedright\arraybackslash}X
        |>{\raggedright\arraybackslash}X |
    }
    \hline
    
    & GBD U5MR & IGME U5MR \\
    
    \hline
    
    Covariates & yes & no \\
    
    \hline
    
    Smoothing Model & Gaussian Process & B-splines \\
    
    \hline
    
    Smoothing hyper-parameters & fixed & estimated \\
    
    \hline
    
    Sampling error & fixed & fixed, estimated \\
    
    \hline
    
    Non-sampling error & fixed & estimated \\
    
    \hline
    
    Systematic bias & no & estimated \\
    
    \hline
\end{tabularx}

==> tables/hierarchical_modeling.tex <==
\begin{tabularx}{1\textwidth}{
        |>{\raggedright\arraybackslash}X
        |>{\raggedright\arraybackslash}X
        |>{\raggedright\arraybackslash}X
        |>{\raggedright\arraybackslash}X
        |>{\raggedright\arraybackslash}X
        |>{\raggedright\arraybackslash}X
        |>{\raggedright\arraybackslash}X
        |>{\raggedright\arraybackslash}X |
    }
    
    \hline
                      & Li 2019       & Alexander 2018     & Cahill 2018 & GBD & Alkema and New 2014 & Alkema 2017 & BMat 2019 \\
    \hline
    
    $g(t, \bm{\alpha}_c)$ parameters & NA & none & shared across countries, nested within region, world & & & NA & \\
    
    \hline
    
    Intercepts & NA & none & & & & shared across countries, nested within region, world & \\
    
    \hline 
    
    Regression coefficients & NA & none & & & & none & \\
    
    \hline
    
    Coefficient for time trends & NA & shared across countries & & & & &\\
    
    \hline
    
    Smoothing parameters & & shared across countries & shared across countries & & shared across countries & shared across countries & $\rho_c = \rho^{(global)}$ \\
    
    \hline
    
    Data bias parameters & & & & & shared across data sources & & \\
    
    \hline
    
    Error variance parameters & & & & & & & \\
    
    \hline
\end{tabularx}

==> tables/process_models.tex <==
\begin{tabularx}{1\textwidth}{
    |>{\raggedright\arraybackslash}X
    |>{\raggedright\arraybackslash}X
    |>{\raggedright\arraybackslash}X
    |>{\raggedright\arraybackslash}X
    |>{\raggedright\arraybackslash}X
    |>{\raggedright\arraybackslash}X
    |>{\raggedright\arraybackslash}X
    |>{\raggedright\arraybackslash}X |
}

    \hline
                      & Li 2019 U5MR       & Alexander 2018 NMR     & Cahill 2018 FP & GBD U5MR & Alkema and New 2014 U5MR & Alkema 2017 MMR &  BMat 2019 \\
    \hline
    
    $\eta_{c,t}$ & & & & & & non-AIDS PM & non-AIDS PM \\
    
    \hline
    
    \multicolumn{8}{|l|}{\textbf{Systematic Component}} \\
    
    \hline
    
    Temporal $g(t, \bm{\alpha}_c)$ & no & no & logistic & no & no & no & no \\
    
    \hline
    
    \multicolumn{8}{|l|}{\textbf{Covariate Component}} \\
    
    \hline
    
    Covariate Model $h(X_{c,t}, \bm{\beta}_c)$ & no & piecewise linear & no & linear mixed-effects & no & $\beta_{c, 0} + \sum_k \beta_{c,k} x_{c,x}$ & $\beta_{c, 0} + \sum_k \beta_{c,k} x_{c,x}$  \\
    
    \hline
    
    Covariates & & U5MR & & LDI, education, HIV & & log(GDP per capita), log(GFR), SAB & log(GDP per capita), log(GFR), SAB \\
    
    \hline
    
    Covariate smoothing & &  & &  & & yes & yes \\
    
    \hline
    
    \multicolumn{8}{|l|}{\textbf{Smoothing Component}} \\
    
    \hline
    
    Smoothing model(s) & RW, ICAR & B-splines (cubic) & AR(1) & Gaussian process (Matérn kernel) & B-splines (cubic) & ARIMA(1, 1, 1) & ARI(1, 1): $\epsilon_{c,t} - \epsilon_{c,t-1} \sim AR(1)$ \\
    
    \hline
    
    Hyper-parameters & estimated & estimated & estimated & fixed & estimated & estimated & estimated \\
    
    \hline
    
    Stationary & no & no & yes & yes & no & no & no \\
    
    \hline
    
    Additional structure & & & & & & & reference year: $\epsilon_{c,1990} = 0$ \\
    
    \hline
    
    Differentiable & nowhere & twice & once & depends on kernel parameters & twice & nowhere? & nowhere? \\
    
    \hline
\end{tabularx}
